Blameless and Optimal Control under Prioritized Safety Constraints

In many resource-limited optimal control problems, multiple constraints may be enforced that are jointly infeasible due to external factors such as subsystem failures, unexpected disturbances, or fuel limitations. In this manuscript, we introduce the concept of blameless optimality to characterize control actions that a) satisfy the highest prioritized and feasible constraints and b) remain optimal with respect to a mission objective. For a general optimal control problem with jointly infeasible constraints, we prove that a single optimization problem cannot find a blamelessly optimal control sequence. Instead, finding blamelessly optimal control actions requires sequentially solving at least two optimal control problems: one to determine the highest priority level of constraints that is feasible and another to determine the optimal control action with respect to these constraints. We apply our results to a rocket landing scenario in which violating at least one safety-induced landing constraint is unavoidable. Leveraging the concept of blameless optimality, we formulate blamelessly optimal controllers that can autonomously prioritize the constraints most critical to a mission.

==> algorithm.tex <==
\section{Blamelessly Optimal Control For Polytopic Safety Sets} \label{sec:algorithm}

% It follows from Theorem~\ref{thm:optimal_blameless} that blamelessness and optimality must be solved for independently. 
Finding the smallest set $\Yset_i$ such that the optimal control problem is feasible entails solving an optimization problem where the objective, $g : \reals^n\mapsto \reals$ is constructed using the safety sets $\Yset_1, \ldots, \Yset_m$. As a result of Theorem~\ref{thm:optimal_blameless}, the objective should have the property that $\Yset_i$, $i = 1,\ldots, m$ are level sets of $g(x_N)$, so that for all $x_N \in \Yset_i$ and all $\hat{x}_N \in \Yset_{i+1}$, $g(x_N) \leq g(\hat{x}_N)$. 

\begin{definition}[Polytopic Safety Sets]
A polytopic safety set $\Yset_i \subset \reals^2$ is defined by the tuple $(\mc{V}_i, A_i, b_i)$, where 
\begin{align*}
    \mc{V}_i &= \{ v_{i1}, \ldots v_{ip} \}, \; v_{ij} \in \reals^2,\\
    A_i &= \bma{ccc} a_{i1} & \cdots & a_{ip} \ema^\trans, \; a_{ij} \in \reals^2,\\
    b_i &= \bma{ccc} b_{i1} & \cdots & b_{ip} \ema^\trans, \; b_{ij} \in \reals
\end{align*}
\end{definition}

Polytopic sets admit two representations. The halfspace representation is
%
\begin{align*}
    \Yset_i = \{x \mid A_ix \leq b_i\}.
\end{align*}
%
The vertex representation is
\begin{equation}\label{eqn:polytope_safety_set}
    \Yset_i = \{x \mid x \in \mbf{conv}(\mc{V}_i)\},
\end{equation}
where $\mbf{conv}(\mc{V}_i)$ is the convex hull of $\mc{V}_i$. One representation can be obtained from the other using vertex or facet enumeration, which has a computation time of {\color{red}O()} in the two-dimensional scenario \cite{Bremner1997_facetenum}. In higher dimensions, $p$ could grow exponentially as a function of dimension. For example, an $d-$dimensional hypercube has $p = 2^d$ vertices.


The objective generation algorithm, Algorithm~\ref{alg:objective_gen}, is illustrated for one-dimensional safety constraints in Figure~\ref{fig:polytope_objective}, and for two-dimensional polytope constraints in Figure~\ref{fig:polytope_objective}. The level sets of the resulting objective function should correspond to the safety sets. The geometry of the constraint sets is therefore exploited in the formation of the objective function, which is generated as a piecewise function. 
%When the safety sets are polytopes, Algorithm~\ref{alg:objective_gen} generates such a function. 
The boundary of $\Yset_i$ is denoted $\delta \Yset_i$.

\begin{algorithm}
\caption{Objective Generation}
\label{alg:objective_gen}
\begin{algorithmic}[1]
\Require $\left\{\Yset_i, \mc{V}_i, \{A_i, b_i\}\right\}_{1\leq i\leq m}$~\eqref{eqn:polytope_safety_set}, $g_0, g_1 \in \reals$.
\Ensure $g:\reals^n \mapsto \reals$. 
% set cost in X1
\State $\mc{S}_0 \coloneqq \Yset_1$, $g(x) \coloneqq g_0, \ \forall \ x \in \mc{S}_0$
% set cost in dX2
\State $g(x) \coloneqq g_1, \ \forall x \in \delta \Yset_2$.
% use min / max distancecs between sets to get costs at each dXi
\For{$i = 2, \ldots, m-1$}
    \State $d_{(i-1)i}^{\min} \coloneqq \min \{ \norm{x-y}_2 \mid x\in\delta\Yset_{i-1}, y\in\delta\Yset_{i} \}$. \label{algline:dmin}
    \State $d_{i(i+1)}^{\max} \coloneqq \max \{\norm{y-z}_2\mid y\in\delta\Yset_{i}, z\in\delta\Yset_{i+1}\}$. \label{algline:dmax}
    \State $g(x) \coloneqq \frac{d_{i(i+1)}^{\max}}{d_{(i-1)i}^{\min}} (g_{i}-g_{i-1}) + g_i$ for all $x\in \delta\Yset_{i+1}$. \label{algline:g_boundary}
\EndFor
% triangulate to get simplices
\For{$i = 1, \ldots, m-1$}
    \State $\{(d_1, d_2, d_3)\} \in \reals^{2\times 3\times r_i} \coloneqq \text{Delaunay}(\mc{V}_{i-1}, \mc{V}_i)$\label{algline:delaunay}
    \For{$j=1,\ldots,r_i$}
    \State \[\bma{c} g(d_1)\\ g(d_2) \\ g(d_3) \ema = \bma{cc} d_1 & 1\\ d_2 & 1 \\ d_3 & 1 \ema \bma{c} \alpha_j \\ \beta_j \ema\]
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth, trim={0cm 0 0cm 0},clip]{figs/objective_1d.eps}
%     \caption{Objective function for one-dimensional constraint sets.}
%     \label{fig:objective_gen}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth, trim={0cm 1.5cm 0cm 1.5cm},clip]{figs/polytope_objective_construction.png}
    \caption{Objective function for two-dimensional polytope constraint sets.}
    \label{fig:polytope_objective}
\end{figure}

Lines~\ref{algline:dmin} and \ref{algline:dmax} can be found by computing the distance from each of the vertices in one set to the hyperplanes making up the neighbouring set, using Algorithm~\ref{alg:dmin_max}. Line~\ref{algline:delaunay} of Algorithm~\ref{alg:objective_gen} performs a Delaunay triangulation, which has a running time of $O(N\log N)$, where $N$ is the number of points being triangulated \cite{Lee1980_delaunay}. A description of the algorithm can be found in \cite{Lee1980_delaunay} and packages implementing the algorithm are readily available \cite{Scipy}. 

\begin{corollary}
Algorithm~\ref{alg:objective_gen} when the $\Yset_i \subset \reals^2$ has a running time of $O(MN\log N)$, where $M$ is the number of safety constraints and $N$ is the number of vertices in two subsequent safety sets.
\end{corollary}

\begin{proof}

\end{proof}

\begin{algorithm}
\caption{Minimum and Maximum Distances}
\label{alg:dmin_max}
\begin{algorithmic}[1]
\Require $\Yset_{i-1}, \Yset_{i}, \Yset_{i+1}$.
\Ensure $d^{\min}_{(i-1)i}, d^{\max}_{i(i+1)}$. 
\For{$v_{(i-1)j} \in \mc{V}_{i-1}$}
    \For{$a_{ik} \in \mc{A}_{i}$}
        \State $d^{\min}_{(i-1)i} = \min\{ d^{\text{min}}_{(i-1)i}, \frac{\abs{a_{ik}^\trans v_{(i-1)j} + b_{ik}}}{\norm{a_{ik}}} \}$
    \EndFor
\EndFor
\For{$v_{(i+1)j} \in \mc{V}_{i+1}$}
    \For{$a_{ik} \in \mc{A}_{i}$}
        \If{$a_{ik}^\trans v_{(i+1)j} \leq b_{ik}$}
            \State \texttt{continue}
        \Else
            \State $d^{\max}_{i(i+1)} = \max\{ ^{\max}_{i(i+1)}, \frac{\abs{a_{ik}^\trans v_{j(i+1)} + b_{ik}}}{\norm{a_{ik}}} \}$
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

The objective resulting from Algorithm~\ref{alg:objective_gen} is a piecewise function in $x \in \reals^2$, of the form
\begin{equation} \label{eq:piecewise_objective}
    g(x) = \begin{cases}
        g_0 & x \in \mc{S}_0\\
        \alpha_1^\trans x + \beta_1 & x \in \mc{S}_1\\
        \vdots\\
        \alpha_R^\trans x + \beta_R & x \in \mc{S}_R
    \end{cases},\,
\end{equation}
% It is straightforward to show that in order to ensure that the objective $g$ is convex, the minimum slope of $g$ between sets $\delta \Yset_2$ and $\delta \Yset_3$ should be greater than or equal to the maximum slope of $g$ between $\delta \Yset_1$ and $\delta \Yset_2$. This requirement dictates the value of the objective at the boundary of $\Yset_3$.
with $\alpha_r \in \reals^2$, $\beta_r \in \reals$, $\mc{S} \subset \reals^2$ for $r=1, \ldots, R$.

Consider set $C$ the point $x$ in the boundary of $C$. The hyperplane $\{y \mid \gamma^\trans y = \gamma^\trans x \}$ is a supporting hyperplane to $C$ at $x$ if $\gamma^\trans y \leq \gamma^\trans x_0$ for all $y\in C$ \cite{Boyd2004}.

\begin{proposition}
    Each of the planes making up $g(x)$ given by \eqref{eq:piecewise_objective} constructed using Algorithm~\ref{alg:objective_gen} is a supporting hyperplane to the image of $g$ under $\reals^2$, $C = \{ (x, g(x)) \mid x \in \reals^2 \}$. \ie for all $r,\; \mc{S}_r,\; x_0\in\mc{S}_r$ 
    \[\bma{cc} \alpha_r^\trans & 1 \ema y \leq \bma{cc} \alpha_r^\trans & 1 \ema^\trans y_0\] for all $x_0 \in \mc{S}_r$, where $y \in C$, and $y_0 = \bma{cc}x_0^\trans & g(x_0)\ema^\trans$.
\end{proposition}

\begin{proof}
\color{red}
Consider the hyperplane 
\begin{align*}
\mc{H}_r &= \{\alpha_r^\trans x + \beta_r \mid x \in \mc{S}_r \subseteq \reals^2 \}\\
&= \{ y \in C \mid \bma{cc}\alpha_r^\trans & -1\ema^\trans y = -\beta_r,\; x \in \mc{S}_r \},
\end{align*}
and the points  $y = (x,g(x))$ with $x \in \mc{S}_r$ and $\hat{y} = (\hat{x}, g(\hat{x}))$ with $\hat{x} \in \mc{S}_{\hat{r}}$. If $S_r \in \Yset_{i+1} \backslash \Yset_{i}$, $\mc{H}_r$ is a supporting hyperplane to $\Yset_i$ and $\Yset_{i+1}$ since it is defined by the vertices of these sets. It follows that
%
\begin{align*}
    \alpha_r^\trans x \geq \alpha_r^\trans \hat{x}
\end{align*}
%
for $x \in \mc{S}_r$ and $\hat{x} \in \mc{S}_{\hat{r}}$. 

We denote the slope of the hyperplane $\mc{H}_r$ in the third dimension as $\gamma_r^3$. It is a function of the value of the function at the boundaries of $\Yset_i$ and $\Yset_{i+1}$, denoted as $g_{}$

If $g(x) \geq g(\hat{x})$, by Line~\ref{algline:g_boundary} of Algorithm~\ref{alg:objective_gen},
%
\begin{align*}
    \gamma_r^3 &= \frac{g_{r+1} - g_r}{d_{(r+1)r}} \geq \frac{g_{r+1} - g_r}{d_{(r+1)r}^{\max}} \\
    &= \frac{1}{d^{\max}_{(r+1)r}} \left( \frac{d^{\max}_{(r+1)r}}{d^{\min}_{r(r-1)}} (g_r - g_{r-1}) + g_r - g_r \right)\\
    &= \frac{1}{d^{\min}_{r(r-1)}} (g_r - g_{r-1}) \geq \frac{1}{d_{r(r-1)}} (g_r - g_{r-1}) = \gamma_{\hat{r}}^3,
\end{align*}
%
so that
\begin{align*}
    \gamma_i^\trans y \geq \gamma_i^\trans \hat{y} \geq \gamma_j^\trans \hat{y}.
\end{align*}
%
Therefore, $\mc{H}_i$ is a supporting hyperplane to the objective.
\end{proof}

\begin{lemma}
The objective $g$ generated by Algorithm~\ref{alg:objective_gen} is convex and equivalent to the piecewise affine function
\[g(x) = \max_{r=1,\ldots, 2m-1} a_r^\trans x - b_r.\]
\end{lemma}

Note that it is only possible to guarantee convexity of the objective function if the safety constraint boundaries do not overlap, meaning that 
%
\begin{align*}
    \delta \Yset_i \cap \delta \Yset_{i+1} = \O, \; \forall i = \{1, \ldots, m-1\}.
\end{align*}

%In the one dimensional case, $g(x)$ can be constructed as a set of piecewise-linear functions. In the two dimensional case, the construction of $g(x)$ is dependent on the shape of the safety constraints. For polytope safety constraints, $g(x)$ can be constructed as a set of piecewise-linear functions. If the safety constraints are ellipses, $g(x)$ is a set of elliptical cones. By assigning the cost at the boundary of a set correctly, the objective can be selected to be convex, provided two safety sets do not share a boundary. {\color{red} expand on this--appendix?}

Using the objective function generated in Algorithm~\ref{alg:objective_gen}, the algorithm for solving for blameless optimality is described in Algorithm~\ref{alg:blamelessopt}.

\begin{algorithm}
\caption{Blameless Optimality}
\label{alg:blamelessopt}
\begin{algorithmic}[1]
% \Require $\Yset_1, \Yset_2, \ldots, \Yset_m$
\State Formulate the objective $g$ using Algorithm~\ref{alg:objective_gen}.
\State Solve
\begin{subequations}
\label{eq:sp1}
\begin{alignat}{3}
&& \min_{u_{1:N|t}} ~& g(x_{N|t}) \label{algline:blameless_objective}\\
&& \st ~& x_{k+1|t} = f(x_{k|t},u_{k|t})\\
&&&u_{k|t} \in \mc U,\; x_{0|t} \in \Xset_0
\end{alignat}
\end{subequations}
\State Use output to determine $\Yset_j$.
\State Solve
\begin{subequations}
\label{eq:sp2}
\begin{alignat}{3}
    && \min_{u_{1:N|t}} ~& q (x, u) \\
    && \st ~& x_{k+1|t} = f(x_{k|t}, u_{k|t}), x_{0|t} = x_0 \in \Xset_0\\
    &&& u_{k|t} \in \Uset,\; x_{N|t} \in \Yset_j
\end{alignat}
\end{subequations}
\end{algorithmic}
\end{algorithm}

The result of \eqref{eq:sp1} is used to determine the highest priority set for which the optimal control problem is feasible. This set is then enforced as a state constraint in the optimal control problem~\eqref{eq:sp2}. Problem~\ref{eq:sp2} can be solved using any optimal control algorithm {\color{red} such as \cite{}.}

\begin{theorem}
Algorithm~\ref{alg:blamelessopt} with the objective in Line~\ref{algline:blameless_objective} generated by Algorithm~\ref{alg:objective_gen}, generates a blameless control sequence and finds the highest priority safety set that is also feasible.
\end{theorem}

\begin{proof}
By construction, the level sets of $g$ are equal to the safety sets $\Yset_i$, $i = 1,\ldots, m$. Suppose the control sequence $u_{1:N|t}$ found by solving Problem~\ref{eq:sp1} is blameworthy, meaning that $x_{N|t} \neq \Yset_i$, and there exists a control sequence $\hat{u}_{1:N|t} \in \Uset$ such that the resulting terminal state $\hat{x}_{N|t} \in \Yset_i$. Then, by construction of $g(x_{N|t})$, $g(x_{N|t}) > g(\hat{x}_{N|t})$ and $\hat{u}_{N|t}$ is a solution to Problem~\ref{eq:sp1}.
\end{proof}


==> introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}
In safety-critical tasks such as  navigating crowded roadways and flying in weather-uncertain air spaces\tc{red}{CITE}, human operators may face safety requirements that are \emph{jointly infeasible}. For example, a helicopter pilot may need to perform an emergency landing in urban spaces and lack the necessary fuel to reach the nearest designated landing zone. In these situations, human operators abide by ethical standards, sacrificing ethically low-priority constraints to ensure higher-priority constraints. For instance, a human pilot may land in an abandoned field risking his or her own life to avoid a endangering the lives of others. Can autonomous systems achieve the same ethical standards?

\begin{problem}\label{prob:intro}
Under jointly infeasible safety constraints, can autonomous algorithms simultaneously 1) prioritize the most ethical safety requirements and 2) optimize mission objectives (e.g. fuel, task completion time)? 
\end{problem}

Problem~\ref{prob:intro} is fundamentally linked to the need for autonomous systems to make ethical decisions~\tc{red}{CITE}. As autonomous technology matures, safety-critical tasks will be gradually offloaded by non-expert human operators to autonomous robots and vehicles. 
Yet without provable ethical guarantees, autonomous systems can not act in ways that do not prioritize ethics and can be blameworthy for making human-interactive environments unsafe.
% Yet without provable ethical guarantees, autonomy is not \emph{trustworthy} and cannot freely operate in human-interactive environments. As a result, Problem~\ref{prob:intro} represents an essential challenge to the integration of autonomy into human society.}
% As autonomous technology advances, non-expert human operators find themselves overseeing 
% Autonomous systems are often capable of making decisions that can directly impact humans. 
% These systems are sometimes placed in situations in which a nominal plan is infeasible due to external circumstances.
% To ensure such systems make decisions that abide by societal standards for ethical practices, autonomous systems should be equipped with alternative plans for such cases. 
% These plans can be ranked in terms of ethicality, 
% For example prioritizing human safety, followed by the protection of property, and of the system itself. Central to handling these plans is an optimization system that can select the safest plan, while still taking into account a mission objective.

This work is concerned with applications in which ethically permissible regions are quantifiable by \emph{state constraints} ranked in order of priority. Blameless autonomy is concerned with scenarios where these regions are not jointly feasible, but instead must be prioritized based on their ethical implications. {\color{violet}For example, when a rocket is landing, the ideal landing zone is a landing pad. If constraints on fuel, system failure, or environmental disturbances prevent the rocket from landing in the desired region, the system should sacrifice environmental integrity first, landing in a region with minor infrastructure that is free of humans. Human safety should only be sacrificed if no other options are available.}

{\color{red} For example, when safely landing an unmanned aerial vehicle (UAV) is infeasible, the autonomous algorithm should first prioritize human safety, followed by environment integrity, and finally followed by UAV integrity. If these constraints are not jointly feasible, the UAV should sacrifice its integrity to prevent environment damage. Likewise, it should sacrifice environmental integrity to ensure human safety.}

% \tc{blue}{We focus on applications in which the safety requirements are quantifiable by \emph{state constraints}. 
% %and can be prioritized based on their ethical impacts. 
% Blameless autonomy is concern with scenarios where these safety constraints are not jointly feasible, but instead must be prioritized based on their ethical implications. 
% For example, when safely landing an unmanned aerial vehicle (UAV) is infeasible, the autonomous algorithm should first prioritize human safety, followed by environment integrity, and finally followed by UAV integrity. If these constraints are not jointly feasible, the UAV should sacrifice its integrity to prevent environment damage. Likewise, it should sacrifice environmental integrity to ensure human safety.}
%{\color{red}This work is concerned with situations in which ethically permissible regions can be defined by state constraints ranked in order of priority. One application of this concept is to the problem of landing a rocket. The ideal landing area is landing pad. If the rocket cannot reach the landing pad due to insufficient fuel, system failure or environmental disturbances, the rocket should land in a region surrounding the landing pad, in which there is risk of damaging infrastructure, but there are no humans. The rocket should only land in the region surrounding this area free of humans and risk harming a person if the two higher priority zones are unreachable. In this situation, it is critical that the rocket land in the highest priority area since landing in lower priority regions risks causing significant damage.}

% This work introduces the concept of blameless optimality, in which safety and ethicality are prioritized, while also optimizing over a mission objective. 
% We show that in general,

If an autonomous system fails to ethically prioritize its safety constraints, we call it \emph{blameworthy}. For instance, if a UAV causes property damage to prevent damage to itself then it is blameworthy for that damage. In contrast, we denote an autonomous system that is not blameworthy as \emph{blameless}. This paper studies the design of blameless autonomous systems and the trade-off between blamelessness and optimality introduced in Problem~\ref{prob:intro}.
% Denoting actions that satisfy the most ethical and feasible safety constraints as \emph{blameless}, we introduce the concept of \emph{blameless optimality} to answer Problem~\ref{prob:intro}. For a class of mission objectives, our results demonstrate that solving} a single optimization problem cannot \tc{blue}{simultaneously optimize mission objectives and guarantee blamelessness.}
% solve for optimality with respect to a mission objective, while simultaneously guaranteeing blamelessness. 
% As such, there is a tradeoff between blamelessness and optimality that requires Problem~\ref{prob:intro} %the blameless optimality problem 
% to be solved \tc{blue}{in two iterations} by solving two subproblems.

\textbf{Contributions}. We provide a precise definition of blameless actions for optimal control problems with ethically prioritized state constraints and related it to control reachable sets. The definition is intended to be widely applicable across various domains. 
% Then, u
Using this definition, we prove that no single optimal control problem with a continuous objective function in its state and control variables can produce a blamelessly optimal action.
% it is shown that blamelessness and optimality cannot, in general, be solved for simultaneously.
Given a sequence of prioritized state constraints, we formulate a triangulation algorithm that generates a \emph{continuous objective function} for a class of prioritized state constraints. We prove that the resulting optimal control problem 1) produces a blameless action and 2) finds the most prioritized and feasible state constraint. We then demonstrate how this algorithm can be used to extend standard optimal control solutions to a two-iteration algorithm that is blameless and optimal. We use our algorithm to answer Problem~\ref{prob:intro} for a real-time rocket landing challenge safety requirements that are jointly infeasible due to fuel limitations.
% Finally, an algorithm for solving the blameless autonomy problem is provided. Results using the proposed algorithm are presented to validate the method.

==> relatedwork.tex <==
\section{Related work}
\label{sec:related work}

The concept of safety in control has been considered using a variety of approaches. Reachability analysis is widely used to guarantee safety properties of dynamical systems \cite{Bansal2017_reachability, Dixit2018_MPCpotentialreach, Leung2020_reachability}. Hamilton-Jacobi (HJ)  reachability is used to verify performance and safety of dynamical systems. A system can pre-emptively avoid sets from which unsafe sets are reachable, or find safe sets of states that are reachable to which it can move \cite{Bansal2017_reachability}. Reachability analysis is used in conjunction with potential field methods in \cite{Dixit2018_MPCpotentialreach} to avoid collisions in autonomous driving. Reachability analysis is used within an optimal control framework in \cite{Leung2020_reachability}. While reachability analysis is applicable to nonlinear systems, can handle control and disturbance variables, and can represent arbitrary shapes, it experiences exponential computational complexity with respect to the number of state variables \cite{Bansal2017_reachability}.

Model predictive control (MPC), solves an optimal control problem over a finite horizon, and applies the first element of this sequence to the agent \cite{Zagaris2018_KOZ_MPC}. Constraints can be enforced within the optimal control problem, however, the minimization of an objective such as fuel consumption or control effort subject to these constraints may lead to infeasibility within the optimization problem. Infeasibility is commonly averted by introducing slack variables \cite{Weiss2015_MPC_soft_constraints}. Other approaches \cite{Vada2001_MPCinfeasibility, Miksch2011_lexicographicMPC} have used lexicographic optimization \cite{Isermann_linlexico} within the context of MPC. Lexicographic optimization is a technique that sequentially optimizes over a finite number of ordered objective functions such that low priority objectives do not interfere with higher priority objectives \cite{Isermann_linlexico}. For a problem with $n$ constraints, finding a solution to the lexicographic optimization problem typically requires solving $n$ problems \cite{Marques_boollexico}. Within the context of MPC, lexicographic optimization has been used to relax constraints in decreasing order or priority when infeasibility arises.

A sampling-based approach to trajectory generation is used in \cite{Starek2017_FMT}, in which the Fast Marching Tree algorithm is used, restricting the growth of trees to a subset of safe samples. Methods for path planning using positive invariant sets have been developed \cite{Danielson2016}. However, these methods are not trivially extended to the case of multiple target zones ranked in order of priority.

\subsubsection*{Notation.}
The state at time step $k$ as computed at time $t$ is denoted $x_{k|t}$. We use the shorthand $x_{1:N|t} $ to denote the sequence of variables $x_{t},\ldots, x_{t+N}$. %Similarly, a sequence of control inputs is denoted $u_{1:N|t} = u_{1|t}, \ldots, u_{N|t}$. 
A sequence of constrained control inputs, $u_{1:N|t} = u_{1|t}, \ldots, u_{N|t}, u_{k|t}\in \Uset$ is denoted $u_{1:N|t} \in \Uset^N$.
The notation $[N]$ is used to denote $\{1,\ldots,N\}$. The convex hull of a finite set $\mc{V} = \{v_1,\ldots, v_k\}\in \reals^K$ is denoted $\conv\{\mc{V}\} = \{\sum_{i=1}^k\alpha_iv_i \ | \ \alpha_i \geq 0, \sum_{i=1}^k\alpha_i = 1, v_i \in \mc{V}, i = 1,\ldots,k\}$.
